Strategies, Benefits and Challenges of App Store-inspired Requirements Elicitation

App store-inspired elicitation is the practice of exploring competitors' apps, to get inspiration for requirements. This activity is common among developers, but little insight is available on its practical use, advantages, and possible issues. This paper aims to study strategies, benefits, and challenges of app store-inspired elicitation, and to compare this technique with the more traditional requirements elicitation interviews. We conduct an experimental simulation with 58 analysts and collect qualitative data. Our results show that: (1) specific guidelines and procedures are required to better conduct app store-inspired elicitation; (2) current search features made available by app stores are not suitable for this practice, and more tool support is required to help analysts in the retrieval and evaluation of competing products; (3) while interviews focus on the why dimension of requirements engineering (i.e., goals), app store-inspired elicitation focuses on how (i.e., solutions), offering indications for implementation and improved usability. Our study provides a framework for researchers to address existing challenges and suggests possible benefits to foster app store-inspired elicitation among practitioners.

==> sections/method_LONG.tex <==
\section(Protocol}
\label{sec:method}




The study can be classified as an \textit{experimental simulation}, in which we want to evaluate the natural behaviour of analysts in a contrived settings~\cite{stol18}, as done in other studies about  interviews~\cite{debnath21,pitts2007improving,bano2019teaching,ferrari2020sapeer}. This allows us to make a more in-depth analysis with respect to surveys, and, at the same time, to consider  human aspects.
The study is exploratory, qualitative, and descriptive, in that it aims to provide a \textit{categorisation} of strategies, benefits and challenges of app store-inspired elicitation. 
To this end, we recruit 58 participants, and we set-up a two-phase process of requirements elicitation. In the first phase,  \textit{interview-based elicitation} (IBE), the analysts perform two interviews with a customer, and then  document the requirements. In the second phase, \textit{app-store inspired elicitation} (ASE), the analysts extend the initial requirements based on similar products retrieved from the app stores. We systematically collect and code analysts' reflections, to produce a list of strategies, benefits and challenges in relation to ASE. Benefits and challenges are also compared with those observed by the analysts in relation to interviews. 

%Furthermore, we correlate the novelty of the produced requirements with the adopted strategies, to understand whether certain ones are more effective than others in producing novel ideas. 

\subsection{Study Participants}
\hl{shorter at least a half}
The requirements analysts are graduate students enrolled in the first or second semester of the MSc in Software Engineering and, at the time of the experiment, were all taking a course on Requirements Engineering. In that course, they have been introduced to elicitation techniques and user stories using very standard teaching material which also included examples from very common systems such as an event ticket store and a bookstore. During the first semesters of the program, students have usually taken, or are taking, an introductory course on software engineering and a course on project management. Elective specialized courses (e.g., User Interaction Engineering and courses on Privacy) are in general taken later in the program. The participants include subjects with professional experience in the software industry.

Most of the students enrolled in the course (80\%)  have already some professional experience. In particular, 48.33\% have intense professional experience. Students in this category have covered a variety of roles including software engineers, developers, consultants, defense contractors, and more.
The other 31.67\% have a less significant professional experience in the field and, after an undergraduate degree in a computing-related discipline, have worked either in close fields or have just research or teaching assistantship experience.
The remaining 20\% of the students are ``career changers'', i.e., students who have an undergraduate degree in a non-computing related discipline, have usually some working experience in their field, and have transitioned to computing through a certificate in which they have learned programming, algorithms, computing foundations, and software engineering. While not computing professionals, because of their path, these students are often very mature and well understand many of the challenges associated with requirements elicitation.

\subsection{Research Questions (RQs)}
The following RQs are addressed in our study. 
\begin{itemize}
    \item \textbf{RQ1:} \textit{What are the strategies adopted for the selection of inspirational products to support ASE?} 
    \item \textbf{RQ2:} \textit{What are the benefits and challenges of ASE?}
    \item \textbf{RQ3:} \textit{What are the differences between ASE and IBE?}
\end{itemize}

%\begin{itemize}
%    \item \textbf{RQ1:} \textit{What are the strategies adopted for the selection of inspirational products to support ASE?} The question aims to categorise the typical strategies used by analysts to select similar apps. To answer the question, we collect the comments provided by the analysts to motivate their selection, and we analyse the data to produce a classification of typical strategies. Furthermore, we provide a frequency analysis, to show the most common strategies.  
%    \item \textbf{RQ2:} \textit{Are the strategies correlated with the novelty of the produced requirements?} The question aims to understand whether there is a relationship between the types of strategies adopted and the degree of novelty of the produced requirements with respect to the  requirements documented after interviews. To answer the question, we compute a novelty score of the ASI requirements, and correlate the score with the adopted strategies. 
%   \item \textbf{RQ2:} \textit{What are the benefits and challenges of ASE?} The question aims to understand what are the advantages of using similar apps to take inspiration for novel requirements, and what are the difficulties encountered by the analysts. To answer the question, we collect the comments of the analysts in this regard.
%    \item \textbf{RQ3:} \textit{What are the differences between ASE and IBE?} This question aims to provide a comparison between the two elicitation styles. To answer the question, we categorise benefits and challenges of interviews, and we  critically analyse the differences with the categorisation in RQ2. 
%\end{itemize}

\begin{figure}[h]
\includegraphics[width=\columnwidth]{img/design.pdf}
\caption{Data Collection and Analysis Procedures.}
\label{fig:design}
\end{figure}

The steps of the data analysis and collection procedure (approved, together with the recruitment process, by the Institutional Review Board of \university{}) are described in the following, and depicted in Fig.~\ref{fig:design}. Tasks are depicted with single margin, while double margin indicates data. Tasks 1---8 concern activities for data collection, while 9---18 are for data analysis. 

 

\subsection{Data Collection}

Tasks 1---5 concern \textit{interview-based elicitation}, including all the activities that go from initial customer ideas until documented requirements. These steps are based on the design of the experiment on elicitation interviews by Debnath \textit{et al.}~\cite{debnath21}. Tasks 6---8 concern \textit{ASE}. 

\textbf{1. Preparation} Analysts are given a brief description of an app to develop and are asked to prepare questions for a customer that they will have to interview to elicit the products’ requirements. The product is an app for the management of a summer camp.
A fictional customer is required to study a set of about 50 user stories for the system, which are regarded as the initial customer ideas for the experiment. The user stories are taken from the dataset by Dalpiaz~\cite{dalpiaz2018}, file \texttt{g21.badcamp.txt}. The use of the same customer for all the interviews is in line with similar experiments, such as \cite{bano2019teaching} and \cite{Pitts2004Stopping}. 
%The brief description has an initial part that describes the company's current practice followed by a set of briefly described needs about 
The user stories concern the following features: (1) managing the information, registration, and activities of the participants, (2) giving the participants' guardians the opportunity to register and follow their children, (3) managing the employees’ performance and schedule, 
(4) communicating with parents and employees, and (5) managing facilities. 


\textbf{2. Interview} 
Each analyst performs a 15 minutes interview with the customer, possibly asking additional questions with respect to the ones that they prepared. The  customer answers their questions based on the set of user stories that describe the product---which are not shown to the analysts, to increase realism. %Overall, the customer is required to stick to the content of the user stories as much as possible. However, he is allowed to answer freely when he does not find a reasonable answer in the user story document, to keep the interview as realistic as possible, and capture novel ideas that emerge in the dialogue. 
The analysts are required to record their interviews, and take notes. 

\textbf{3. Requirements Analysis}
Based on the recording and their notes, the analysts have to: (a) perform an initial analysis of the requirements, and based on this analysis (b) produce additional questions for the customer to be asked in a follow-up interview. 
%The initial analysis can be performed with the support of a graphical prototype, use cases, or written form. Analysts can adopt the method they find more suitable.

\textbf{4. Follow-up Interview}
Then, they perform a follow-up interview with the customer, which also lasts 15 minutes, to ask the additional questions prepared. 
%During the interview, they can use the graphical prototype, the use cases, or any material produced as a support to ask questions to the customers. In practice, they can show the material to the customer and discuss based on the material. 

\textbf{5. Requirements Documentation}
After the second interview, they are required to write down from 50 to 60 user stories for the system. We constrain the number of user stories between 50 and 60 to be consistent with the number of user stories in the original set. About 50 user stories are also the typical number in the dataset by Dalpiaz~\cite{dalpiaz2018}, which we deem representative of user story sets used for research purposes.

\textbf{6. Analysis of App Stores}
Each analyst starts from the user stories that they developed in the previous phase. They are now asked to produce an enhanced set of user stories, which take into account possible competing products available on the market. 
%, as commonly done by app developers~\cite{al2019app}. 
%The analysts are asked to imagine that the product is now already developed, and that now they want to sell the product to a wider market. Therefore, they will have to enhance the list of user stories so that the needs of different users can be fulfilled. 
To this end, the analysts are required to perform an informal market analysis based on the app stores. In particular, they are required to:

\begin{itemize}
    \item Select at least 5 mobile apps from Google Play or the Apple App Store that are in some way related to the developed product (for example apps for summer camps, apps for trekking, or anything that they consider related).
    \item  Try out the apps to have an idea of their features when compared with their product. 
    \item Go through the app reviews to identify desired features, and additional requirements that may be appropriate also for their product. 
\end{itemize}

No automated tool, except for the default app store search engines, was provided for the market analysis task. The analysts were free to browse the app stores following their intuition, ability and preferred strategy. The goal was to avoid confounding factors, i.e., the usage of a tool, and also to elicit challenges which could be addressed through---possibly existing---tools. 
Based on the analysis of the app stores, the analysts are required to list the selected apps and their links, together with a brief description that 1. outlines the main features of the product, 2. explains in which way the product is related to the original one, and why they have chosen it.

\textbf{7. Requirements Extension}
Analysts are asked to add 20 user stories to the original list, based on the analysis of the app stores. 

\textbf{8. Reflections}
The analysts are asked to fill a questionnaire to reflect on the experience. This includes of the following open-ended questions: q1) What are the benefits and challenges of app store-inspired elicitation? q2) What are the benefits and challenges of interview-based elicitation?  q3) What are the differences between interview-based and app store-inspired elicitation?

\subsection{Data Analysis}
\hl{specify which guidelines exactly for thematic analysis}
Data analysis is performed by two researchers, r1 and r2, by means of thematic analysis~\cite{braun2006using,cruzes2011recommended}, and following the guidelines by Salda{\~na} for the coding activity~\cite{saldana2021coding}. 
In the following, we report the analysis performed for each RQ. The analysis is generally composed of a first open coding activity made by r1 on a set of 30 analyst, and a complementary procedure carried out by r2 with closed coding on the remaining 28 analysts, using the codes produced by r1. A partial exception is RQ3, for which a brainstorming activity was also included to produce an analysis of the differences between elicitation styles. In addition, for RQ2, we also complemented the analysis with a literature review. 

\paragraph{RQ1} Steps are as follows. 
\hl{I think we can reduce the procedures as it is really boring, and put them in the appendix, and provide only a general description of thematic analysis here (also, modify picture).}

\textbf{9. Strategy Extraction} The input data are the brief descriptions of apps with motivations for the choice, from step 7. The data from the first 30 analysts include 153 items, one for each app. These were inspected by r1, who performed a first open coding round, and identified a set of 9 common strategies. For example a statement such as \textit{This app is related to my app because it is a resource for people who are interested in camping and other outdoor events and activities} was coded as \textit{user profile similarity}. r1 redacted a codebook including: name of the strategy; description; example cases. Based on the codebook, r1 then inspected again each data item, and coded it with a maximum of three strategies (closed coding). We considered this number sufficient to characterise the items, based on the previous analysis. 

\textbf{10. Complementary Procedure} r2 used the codebook to inspect the data from the remaining 28 analysts, 142 items, again coding them with a maximum of three strategies (closed coding). r2 suggested 2 additional strategies, and added it to the codebook. r1 revised his data to account for the additional input. r1 and r2 used the updated codebook and went through each others' coded data for cross-checking. Agreement was evaluated with Cohen's kappa~\cite{landis1977measurement}, resulting in 0.77 (substantial agreement). Final decisions on controversial cases were made in a final meeting. This analysis produced: a codebook with 11 coding strategies, plus, for each item in the data produced by the analysts, a list of strategies used.  

\paragraph{RQ2} Steps are as follows. 

\textbf{11. Benefits/Challenges Extraction} The input data are the reflections from step 8, answers to q1. r1 analysed the answers, and used open coding (two iterations) to identify benefits and challenges. For example the item containing the text \textit{getting hands-on experience with potential features and evaluating their implementation} was coded among benefits as \textit{hands-on evaluation}. Instead, \textit{User reviews are a majority either based on total hatred of a product or complete satisfaction. These two extremes do not lead to productive identification of what requirements are missing in a product.} was coded among challenges as \textit{polarised reviews}. Then, r1 merged similar codes, aggregated them into common categories, and produced two codebooks, one for benefits, and one for challenges, with: category; benefit/challenge; description; examples. Concerning the aggregation into categories, challenge-related codes such as \textit{poor reviews}, \textit{polarised reviews} and \textit{too many reviews} were aggregated into the \textit{Reviews} category.  

\textbf{12. Complementary Procedure I} r2 used the codebooks to annotate the data from the remaining 28 analysts (closed coding). She suggested \hl{X} benefits, \hl{Y} more challenges, and one additional category for benefits, which were added to the codebooks. These represents the final output of the analysis. The codebooks were not used for a further round of closed coding, as we are not interested in frequency analysis. \hl{decide if we should do this, I have to tag...}
%, but rather in eliciting as more benefits and challenges as possible. 

\textbf{13. Complementary Procedure II} to complement benefits and challenges of ASE, we performed a lightweight systematic literature review (SLR) following the guidelines by Kitchenham~\cite{kitchenham2004procedures}.  Specifically, we queried the Scopus engine with the following string (( benefit*  OR  challenge*)  AND  ( (app  AND  store*)  OR  (app  AND  review*)) on title, abstract and keywords, selecting only the Computing area of research, and specific venues (e.g., IEEE TSE, Springer EMSE). The full string is available in our supplementary material. The Scopus database contains peer-reviewed publications from top SE journals and conferences, including IEEE Xplore, ACM Digital library, ScienceDirect (Elsevier), and Springer research papers. Scopus’ coverage is considered optimal when compared to these other databases~\cite{martinez2022software}. The highly selective search string identified 82 publications. We set a main inclusion criterion as \textit{The paper mentions one or more benefits or challenges of app store analysis}. After screening the papers based on this criterion, we finally selected 35 items. These were analysed in detail by r1, to extract further benefits and challenges that could be applied to ASE. The procedure led to an additional set of 1 benefit, and 8 challenges. 

\paragraph{RQ3} 
The input data are reflections from step 8, answers to q2 and q3. Steps are as follows. 

\textbf{14-15. Ben/Chall Extraction \& Compl. Proc.}
An analysis analogous to the one described for RQ2 was carried out on the answers to q2, to produce two codebooks with benefits and challenges of IBE. The complementary procedure for these codebooks led to 8 benefits, and 5 more challenges, within the existing categories. 

\textbf{16. Differences Extraction I} r1 and r2 jointly analysed the codebooks for ASE and IBE (four codebooks). The goal was to produce a first comparative table, contrasting the characteristics of ASE and IBE. For each item in each codebook of an elicitation style, they brainstormed on possible differences with the other style. For example, in relation to the challenge for interviews previously coded as \textit{difficult preparation}, the researchers added the contrasting code \textit{limited preparation needed} for ASE. The codes were then homogenised, and this led to a table with \hl{Y} comparative items.

\textbf{17. Differences Extraction II} To further enrich the table, r1 analysed the answers to q3 for the first 30 analysts, and performed open coding. 
%, to produce a first comparative table, contrasting the characteristics of ASI and IBE.
For example, the sentence \textit{interviews are designed to elicit what the stakeholder wants, and product-inspired elicitation is designed to elicit what the stakeholder potentially didn't know he wanted or needed} led to two contrasting items: (ASE) \textit{identify what the stakeholder could need} vs (IBE) \textit{identify what the stakeholder wants}. This led to an additional set of 14 differences. 

\textbf{18. Complementary Procedure} r2 analysed the remaining 28 analysts with closed coding.
The analysis did not lead to additional items.%The codes were then homogenised by the two researchers with the previously identified differences, but the analysis did not lead to additional items.

%\hl{should be complemented with a literature review: (benefit* OR challenge*) AND (app store* OR app review*) in Scopus. 82 papers identified, restricted to conference, article a and reviews, and limit to certain conference and journals}

%\hl{
%TITLE-ABS-KEY ( ( benefit*  OR  challenge* )  AND  ( ( app  AND  store* )  OR  ( app  AND  review* ) ) )  AND  ( LIMIT-TO ( SUBJAREA ,  "COMP" ) )  AND  ( LIMIT-TO ( DOCTYPE ,  "cp" )  OR  LIMIT-TO ( DOCTYPE ,  "ar" )  OR  LIMIT-TO ( DOCTYPE ,  "re" ) )  AND  ( LIMIT-TO ( EXACTSRCTITLE ,  "ACM International Conference Proceeding Series" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Conference On Human Factors In Computing Systems Proceedings" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Proceedings International Conference On Software Engineering" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "IEEE Transactions On Software Engineering" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Information And Software Technology" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Empirical Software Engineering" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Journal Of Systems And Software" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Expert Systems With Applications" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "IEEE Transactions On Mobile Computing" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "International Symposium On Empirical Software Engineering And Measurement" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Proceedings 2017 IEEE ACM 4th International Conference On Mobile Software Engineering And Systems Mobilesoft 2017" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Proceedings International Conference On Mobile Software Engineering And Systems Mobilesoft 2016" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Proceedings Of The ACM On Human Computer Interaction" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "ACM Transactions On Software Engineering And Methodology" )  OR  LIMIT-TO ( EXACTSRCTITLE ,  "Automated Software Engineering" ) )  }



%The following data are used as source for the analysis, in relation to RQs. \textbf{RQ1:} brief descriptions of apps and motivations for the choice, from step 7. \textbf{RQ2:} reflections from step 8, answers to q1). \textbf{RQ3:} reflections from step 8, answers to questions 2) and 3). 


